Dispersive Evaluation of the Inner Radiative Correction in Neutron and Nuclear $\beta$-decay

We propose a novel dispersive treatment of the so-called inner radiative correction to the neutron and nuclear $\beta$-decay. We show that it requires knowledge of the parity-violating structure function $F_3^{(0)}$ that arises from the interference of the axial vector charged current and the isoscalar part of the electromagnetic current. By isospin symmetry, we relate this structure function to the charged current inelastic scattering of neutrinos and antineutrinos. Applying this new data-driven analysis we obtain a new, more precise evaluation for the universal radiative correction $\Delta_{R}^{V,\,new}=0.02467(22)$ that supersedes the previous estimate by Marciano and Sirlin, $\Delta_R^V=0.02361(38)$. The substantial shift in the central value of $\Delta_R^V$ reflects in a respective shift of $V_{ud}$ and a considerable tension in the unitarity constraint on the first row of the CKM matrix which is used as one of the most stringent constraints on New Physics contributions in the charged current sector. We also point out that dispersion relations offer a unifying tool for treating hadronic and nuclear corrections within the same framework. We explore the potential of the dispersion relations for addressing the nuclear structure corrections absorbed in the ${\cal F}t$ values, a crucial ingredient alongside $\Delta_R^V$ in extracting $V_{ud}$ from superallowed nuclear decays.

==> appDIS.tex <==
Recall that we have expressed the vector-axial inference contribution to the $\gamma W$ box diagram in terms of the $Q^2$-integral over the first Nachtmann moment of the P-odd structure function $F_3^{(0)}$.
The dominant contributor to the integral lies in the large-$Q^2$ regime because the integral scales as $\ln (M_W^2/\Lambda^2)$ where $\Lambda$ is an effective infrared cutoff to the $Q^2$-integration. Fortunately at high-$Q^2$ one enters the DIS regime and the behavior of the first Nachtmann moment is quite well-understood as pQCD applies. Therefore we shall isolate the high-$Q^2$ piece:
\begin{equation}
\Box^{VA,\mathrm{DIS}}_{\gamma W}=\frac{3\alpha}{2\pi}\int_{\Lambda^2}^\infty\frac{dQ^2M_W^2}{Q^2\left[M_W^2+Q^2\right]}M_3^{(0)}(1,Q^2)
\end{equation}
and study its behavior separately.

When $\Lambda^2\gg M^2$, the first Nachtmann moment reduces effectively to the first Mellin's moment:
\begin{equation}
M_3^{(0)}(1,Q^2)\rightarrow \int_0^1dxF_3^{(0)}(x,Q^2)
\end{equation}
where $x=Q^2/(2M\nu)$ is the Bjorken variable. In the parton model the structure function $F_3^{(0)}$ depends on a combination of PDF's
\beqn
F_3^{(0)}(x)=\frac{e_u+e_d}{8}(d_n(x)-\bar u_n(x)).
\eeqn
Assuming further a symmetric sea in the neutron, $\bar u_n=\bar d_n$, the integral over $x$ simply gives the number of valence $d$-quarks inside the neutron (or equivalently, the number of valence $u$-quark inside the proton), $\int_0^1dx(d_n(x)-\bar d_n(x))=\int_0^1dxd_V(x)=2$, and we obtain the large logarithm term already obtained by MS:
\beqn
\Box_{\gamma W}^{VA,\rm DIS}&\approx&\frac{3\alpha}{2\pi}\frac{e_u+e_d}{4}\ln\frac{M_W^2}{\Lambda^2}=
\frac{\alpha}{4\pi}\ln\frac{M_W}{\Lambda},
\eeqn
An important result from Ref. \cite{Marciano:2005ec} was to realize that all pQCD corrections to this leading logarithm term are identical to those entering Bjorken sum rule for polarized electroproduction. These corrections modify the leading log (LL) result for the MS function $F(Q^2)$,
\beqn
&&F^{LL}(Q^2)=\frac{1}{Q^2}\label{eq:pQCD}\\
&&F^{\rm pQCD}=\frac{1}{Q^2}
\left[1-\frac{\bar\alpha_s}{\pi}-C_2\left(\frac{\bar\alpha_s}{\pi}\right)^2-C_3\left(\frac{\bar\alpha_s}{\pi}\right)^3
\right],\nn
\eeqn
with $C_2=4.583-0.333 N_F$ and $C_3=41.440-7.607N_F+0.177N_F^2$, $N_F$ standing for the number of effective quark flavors, 
and $\bar\alpha_s(Q^2)$ denotes the running strong coupling constant in the modified minimal subtraction scheme. 
Numerically, the pQCD corrections reduce the large logarithm $\ln(M_W/\Lambda)\approx3.98$ by roughly 8 \%.


==> appQE.tex <==
In this appendix we provide details of the calculation for the modification of the Born contribution to $F_3$ due to binding effects and Fermi motion in a nucleus. 

%First, realizing that all the superallowed $\beta$-decays considered in the determination of $V_{ud}$ are actually $\beta^+$ decay, it is instructive to first study the amplitude of the ``free" proton decay $p\rightarrow ne^+\nu_e$ despite that it is in fact kinematically prohibited. In analogy to Eq. \eqref{eq:BoxgaW}, the tree-level and the $V\times A$ contribution from the $\gamma W$ box-diagram to the Fermi amplitude of the proton $\beta^+$ decay can be written as:
%\begin{equation}
%T^{p}_{W}+T^{VA,p}_{\gamma W}=-\sqrt{2}G_FV_{ud}\left[1+\Box^{VA,p}_{\gamma W}\right]\bar u_\nu\pdagger(1-\gamma_5) v_e,
%\end{equation}
%and one may straightforwardly demonstrate that
%\begin{equation}
%\Box^{VA,p}_{\gamma W}=4\pi\alpha\mathrm{Re}\int\frac{d^4q}{(2\pi)^4}\frac{M_W^2}{M_W^2+Q^2}\frac{Q^2+\nu^2}{Q^4}\frac{T_3^{(0),p}(\nu,Q^2)}{M\nu},
%\end{equation}
%with the form identical to Eq. \eqref{eq:boxexplicit}. The function $T_3^{(0),p}(\nu,Q^2)$ is the parity-odd spin-independent invariant amplitude involving $J_{em}^{(0)\mu}$, namely the isosinglet component of the electromagnetic current, in the following forward Compton tensor:
%\beqn
%T^{\mu\nu}_{\gamma W,p}=\int dxe^{iqx}\langle n|T[J^\mu_{em}(x)\left(J^{\nu}_W(0)\right)^\dagger]|p\rangle.
%\eeqn
%Next, by isospin symmetry one can show that:
%\begin{equation}
%\left\langle p\right|J_{em}^{(0)\mu} J_W^\nu\left|n\right\rangle=\left\langle n\right|J_{em}^{(0)\mu} \left(J_W^\nu\right)^\dagger\left|p\right\rangle.
%\end{equation}
%From the result above one immediately deduces that $T_3^{(0),p}=T_3^{(0)}$, i.e. $\Box_{\gamma W}^{VA,p}=\Box_{\gamma W}^{VA}$. So what we studied here for the neutron beta decay can be directly applied to case of the $\beta^+$ decay of proton.

We start by approximating the full nuclear Green's function by the subset with one active nucleon and a nuclear spectator, also known as the plane wave impulse approximation (PWIA). We write for the initial state $|A\rangle$ and final state $|A'\rangle$ wave functions involved in a $\beta^+$ decay process,
\beqn
|A\rangle&=&\sqrt{2E_A}\sum_{p\in A}\int\frac{d^3\vec k \phi^p_A(k)|p(\vec k),A-p(-\vec k)\rangle}{(2\pi)^3\sqrt{2E_{A-1}\,2E_n}}\\
|A'\rangle&=&\sqrt{2E_{A'}}\sum_{n\in A'}\int\frac{d^3\vec k \phi^n_{A'}(k)|n(\vec k),A'-n(-\vec k)\rangle}{(2\pi)^3\sqrt{2E_{A-1}\,2E_n}},\nn
\eeqn
with the on-shell condition for the intermediate nuclear state $A-p=A'-n$ but in general off-shell active nucleon with a 3-momentum $\vec k$. The momentum distribution function is normalized according to
\beqn
\int\frac{d^3\vec k}{(2\pi)^3}|\phi(k)|^2=1, 
\eeqn
while the nuclear state normalization is 
\beqn
\langle A(\vec k)|A(\vec k')\rangle=(2\pi)^32E_A\delta^3(\vec k-\vec k').
\eeqn

The $\gamma W$ interference Compton tensor in the $\beta^+$ decay of a nucleus $A$ can be defined as
\beqn
T^{\mu\nu}_{\gamma W,A}=\int dxe^{iqx}\langle A'|T[J^\mu_{em}(x)\left(J^{\nu}_W(0)\right)^\dagger]|A\rangle.
\eeqn
Using the above definitions we arrive to
the following expression in PWIA:
\beqn
T_{\gamma W,A}^{\mu\nu}&=&\sum_{p\in A}\int\frac{d^3\vec k}{(2\pi)^3}(\phi^n_{A'}(k))^*\phi^p_A(k)T_{\gamma W,p}^{\mu\nu}.
\eeqn
We aim at a universal correction that only takes into account the bulk nuclear properties, not the fine details of each initial and final nucleus. To this precision we assume that the momentum distribution of protons in the initial nucleus and neutrons in the final nucleus are the same, $\phi^p_{A'}(k)=\phi^n_A(k)=\phi(k)$. This assumption is natural, e.g. in the Fermi gas model of nucleus that we shall describe later. We then obtain a master formula in PWIA:
\beqn
T_{\gamma W,A}^{\mu\nu}(P,q)=\sum_{p\in A}\int\frac{d^3\vec k}{(2\pi)^3}|\phi(k)|^2T_{\gamma W,p}^{\mu\nu}(k,q),\label{eq:PWIA}
\eeqn
with the nuclear momentum taken at rest, $P^\mu=(M_A,\vec0)$. The Compton tensor $T^{\mu\nu}_{\gamma W,A}$ can be decomposed in terms of invariant functions as in Eq. \eqref{eq:Wmunu}, and we are interested in the P-odd invariant function $T_{3,A}^{(0)}$. 

It is informative to consider the limit of non-interacting nucleons (nucleon tensor independent of $k$) where we obtain
\beqn
T_{\gamma W,A}^{\mu\nu}&=&\sum_{p\in A}T_{\gamma W,p}^{\mu\nu}.
\eeqn
The relation Dis$T_i=4\pi F_i$ holds for each target with the respective mass. The nucleus is considered at rest, and neglecting nucleon recoil corrections $\sim\vec k^2/M^2$ we obtain for the structure function of interest,
\beqn
F_{3,A}^{(0)}&=&\sum_{p\in A}F_{3,p}^{(0)}.\label{eq:F3An}
\eeqn
In the limit of non-interacting nucleons, the nuclear structure function scales as the number of protons, just like the tree-level vector coupling of the $W$ boson to the nucleus. This confirms the result of Marciano and Sirlin for $C_B$ obtained in the free nucleon limit.

We now want to go beyond this limit by using Eq. (\ref{eq:PWIA}) to obtain: 
\beqn
F_{3,A}^{(0)}(P\cdot q,Q^2)=\sum_{p\in A}\int\frac{d^3\vec k}{(2\pi)^3}|\phi(k)|^2F_{3,p}^{(0)}(k\cdot q,Q^2).\nn
\eeqn
Here we are interested in the quasielastic contribution to $F_{3,A}^{(0)}$ which results from the smearing of the elastic term of the free proton. The latter can be inferred from Eq. \eqref{eq:F3Born}:
\beqn
&&F_{3,p}^{(0),B}(k\cdot q,Q^2)=F_{3}^{(0),B}(k\cdot q,Q^2)\\
&&=-\frac{Q^2}{4}G_A(Q^2)G_M^S(Q^2)\delta((k+q)^2-M^2).\nn
\eeqn
To perform the integral over $d^3\vec k=k^2dk d\cos\theta d\phi$ we choose the $z$-axis along the direction of the virtual photon, $q^\mu=(\nu,0,0,q)$ with $\nu=(P\cdot q)/M_A$ and $q=\sqrt{\nu^2+Q^2}$. 
The $\phi$ integration is trivial, while the $\delta$-function removes that over $d\cos\theta$ via 
\beqn
\delta((k+q)^2-M^2)=\frac{1}{2kq}\delta(\cos\theta-\cos\theta_k),
\eeqn
with
\beqn
&&\cos\theta_k\\
&&=\frac{(M_A+\nu)^2-2(M_A+\nu)p_{A-1}+M_{A-1}^2-M^2-\vec q^2}{2kq},\nn
\eeqn
with $p_{A-1}=\sqrt{M_{A-1}^2+\vec k^2}$ the energy of the on-shell spectator. One is left with an integral over $k=|\vec k|$ to obtain the quasielastic contribution to $F_{3,A}^{(0)}$:
\beqn
F_{3,A}^{(0),QE}(\nu,Q^2)=-\sum_{p\in A}G_AG_M^S\frac{Q^2}{32\pi^2q}
\int\limits_{k_-}^{k_+} kdk|\phi(k)|^2.\nn\\
\eeqn
Requiring that $-1\leq\cos\theta_k\leq1$ yields the upper and lower limits of $k$ as shown in Eq. \eqref{eq:kpm} upon neglecting terms of order $\epsilon/M_A$. 
Thus, for the initial nucleus with $Z$ protons we obtain:
\beqn
F_{3,A}^{(0),QE}(\nu,Q^2)=-ZG_AG_M^S\frac{Q^2}{16q} \langle\frac{1}{k}\rangle(\nu,Q^2),
\eeqn
with the average inverse nucleon momentum defined as
\beqn
\langle\frac{1}{k}\rangle(\nu,Q^2)=\int\limits_{k_-(\nu,Q^2)}^{k_+(\nu,Q^2)} \frac{kdk}{2\pi^2}|\phi(k)|^2.
\eeqn

As an exploratory model we consider the free Fermi gas model that corresponds to a uniform momentum distribution inside the sphere with the  radius equal to the Fermi momentum $k_F$
\beqn
\frac{1}{(2\pi)^3}|\phi(k)|^2=\frac{3}{4\pi k_F^3}\theta(k_F-|\vec k|),
\eeqn
resulting in 
\beqn
\langle\frac{1}{k}\rangle(\nu,Q^2)&=&\frac{3\left((\tilde k_+)^2-(\tilde k_-)^2\right)}{2 k_F^3},
\eeqn
with $\tilde k_\pm=\mathrm{min}(k_\pm,k_F)$.
Finally, we account for Pauli blocking by means of the function
\beqn
F_P(|\vec q|,k_F)=\frac{3|\vec q|}{4k_F}\left[1-\frac{\vec q^2}{12k_F^2}\right]\;\;\;{\rm for}\;\;|\vec q|\leq2k_F,
\eeqn
and $F_P=1$ otherwise. With these we obtain $F_{3,A}^{(0),QE}$ per proton for $\beta^+$ decay of a heavy nucleus as:
\beqn
\frac{1}{Z}F_{3,A}^{(0),QE}(\nu,Q^2)=-G_AG_M^S\frac{3Q^2}{32q}F_P\frac{\left((\tilde k_+)^2-(\tilde k_-)^2\right)}{k_F^3}.\nn\\
\eeqn


==> appborn.tex <==
This appendix serves as an updated evaluation of the elastic contribution to the $\gamma W$ box diagram. As clearly seen from Fig. \ref{fig:spectrum} the elastic contribution is separated from inelastic one by a finite gap. This picture remains intact for any value of $Q^2$, so it is natural to separate this piece out of the integral. To evaluate it, we need electromagnetic and weak vertices. 
The electromagnetic vertex is given by
\beqn
\Gamma_{em}^{\mu}(q)&=&\left[F_1^S(Q^2)\frac{\mathbbm{1}}{2}+F_1^V(Q^2)\frac{\tau^3}{2}\right]\gamma^\mu\\
&+&\left[F_2^S(Q^2)\frac{\mathbbm{1}}{2}+F_2^V(Q^2)\frac{\tau^3}{2}\right]i\sigma^{\mu\alpha}\frac{q_\alpha}{2M},\nn
\eeqn
with $F_{1,2}^{S,V}=F_{1,2}^p\pm F_{1,2}^n$ and $q$ the incoming momentum. The weak charged current vertex is given by
\beqn
\Gamma_W^{a,\mu}(q)=\left[F_1^W\gamma^\mu+F_2^Wi\sigma^{\mu\alpha}\frac{q_\alpha}{2M}+G_A\gamma^\mu\gamma_5\right]\tau^a;
\eeqn
here we do not display the pseudoscalar form factor $G_P$ that does not contribute to the box diagram. 

A straightforward calculation leads to the following expression for the elastic contribution to the structure function,
\beqn
F_{3,\,\rm Born}^{(0)}=-\frac{1}{4}G_A(Q^2)G_M^S(Q^2)\delta(1-x)\label{eq:F3Born}
\eeqn
where $G_M^S=F_1^S+F_2^S$ is the isoscalar magnetic Sachs form factor. The resulting contribution to the box correction reads
\begin{eqnarray}
\Box_{\gamma W}^{VA,\mathrm{Born}} &=&  -\frac{\alpha}{\pi }\int\limits_{0}^{\infty}dQ\frac{2\sqrt{4M^{2}+Q^{2}}+Q}{\left(\sqrt{4M^{2}+Q^{2}}+Q\right)^{2}}\nn\\
&&\times G_{A}(Q^{2})G_{M}^{S}(Q^{2})
\end{eqnarray}
Above, we neglected the $Q^2$-dependence of the $W$-propagator since the integral converges way below $Q^2\sim M_W^2$ due to nucleon form factors. Notice that unlike Marciano and Sirlin who only account for the elastic contribution in the low-$Q^2$ part of the integral, in the dispersive approach it extends to all $Q^2$. 


Numeric evaluation with modern data on electromagnetic and weak form factors leads to
\beqn
\Box_{\gamma W}^{VA,\rm Born}=\frac{\alpha}{2\pi}0.908(49)=1.05(6)\times 10^{-3},\label{eq:Bornvalue}
\eeqn
slightly above the MS value \cite{Marciano:2005ec},
\beqn
\Box_{\gamma W}^{VA,\rm Born}\Bigr|_{\mathrm{MS}}=\frac{\alpha}{2\pi}0.829(83)=9.63(96)\times 10^{-4}.
\eeqn
The two calculations agree within the errors, but the uncertainty in the MS calculation is rather arbitrarily assigned as $\pm 10\%$, whereas ours is derived from the most recent information on nucleon form factors and is half of that in MS. This result is essentially model-independent: form factors are fixed by data on electron and neutrino scattering. If future data will further constrain the form factors, the uncertainty can be further reduced. 

In the following we present the details in obtaining the Born contribution \eqref{eq:Bornvalue} to $\Box_{\gamma W}$. First, we notice that according to our definitions, $G_{M}^{p}(Q^{2})>0$,
$G_{M}^{n}(Q^{2})<0$, $G_{A}(Q^{2})<0$ and $|G_{M}^{p}(Q^{2})|>|G_{M}^{n}(Q^{2})|$
for all relevant values of $Q^{2}$. So, we can write $\Box_{\gamma W}^{VA,\mathrm{Born}}$ 
as:
\beqn
\Box_{\gamma W}^{VA,\mathrm{Born}}&=&\frac{\alpha}{\pi}\int_0^\infty dQ\frac{2\sqrt{4m_{N}^{2}+Q^{2}}+Q}{\left(\sqrt{4m_{N}^{2}+Q^{2}}+Q\right)^{2}}\\
&\times&|G_{A}(Q^{2})|\left(|G_{M}^{p}(Q^{2})|-|G_{M}^{n}(Q^{2})|\right),\nn
\eeqn
so that every single multiplicative term in the integrand is positive
definite.

We acquire the data of the nucleon magnetic Sachs form factors from Fig. 1
and Fig. 4 of Ref. \cite{Ye:2017gyb}.
In each figure, we take the upper and lower boundary of the red shaded
band (multiplied by appropriate factors) as our $|G_{M}^{N}(Q^{2})|_{\mathrm{max}}$
and $|G_{M}^{N}(Q^{2})|_{\mathrm{min}}$ respectively ($N=p,n$),
and define:
\begin{eqnarray}
|G_{M}^{N}(Q^{2})| & = & \frac{1}{2}\left(|G_{M}^{N}(Q^{2})|_{\mathrm{max}}+|G_{M}^{N}(Q^{2})|_{\mathrm{min}}\right)\nonumber \\
\Delta|G_{M}^{N}(Q^{2})| & = & \frac{1}{2}\left(|G_{M}^{N}(Q^{2})|_{\mathrm{max}}-|G_{M}^{N}(Q^{2})|_{\mathrm{min}}\right).\nn\\
\end{eqnarray}

For the axial form factor at low $Q^{2}$, we utilize the result from
the model-independent $z$-expansion analysis in Ref. \cite{Bhattacharya:2011ah}. We take the upper and lower
end of the green error bars in their Fig. 3 as our $|G_{A}(Q^{2})|_{\mathrm{max}}$
and $|G_{A}(Q^{2})|_{\mathrm{min}}$, and define $|G_{A}(Q^{2})|$
and $\Delta|G_{A}(Q^{2})|$ accordingly. For $Q^{2}>1$ GeV$^{2}$,
we extrapolate each of the upper and lower curve using a dipole function
$g_{A}(1+Q^{2}/m_{A}^{2})^{-2}$ with $g_A\approx 1.27$. We find that, for a smooth exctrapolation
of $|G_{A}(Q^{2})|_{\mathrm{max}}$ we need $m_{A}=1.27$ GeV while
for $|G_{A}(Q^{2})|_{\mathrm{min}}$ we need $m_{A}=1.09$ GeV. 

For the uncertainty estimation, we define:
\begin{widetext}
\begin{eqnarray}
\delta_1 & = & \frac{\alpha}{\pi}\int_0^\infty dQ\frac{2\sqrt{4m_{N}^{2}+Q^{2}}+Q}{\left(\sqrt{4m_{N}^{2}+Q^{2}}+Q\right)^{2}}\Delta|G_{A}(Q^{2})|\left(|G_{M}^{p}(Q^{2})|-|G_{M}^{n}(Q^{2})|\right)\nonumber \\
\delta_2 & = & \frac{\alpha}{\pi}\int_0^\infty dQ\frac{2\sqrt{4m_{N}^{2}+Q^{2}}+Q}{\left(\sqrt{4m_{N}^{2}+Q^{2}}+Q\right)^{2}}|G_{A}(Q^{2})|\left(\Delta|G_{M}^{p}(Q^{2})|\right)\nonumber \\
\delta_3 & = & \frac{\alpha}{\pi}\int_0^\infty dQ\frac{2\sqrt{4m_{N}^{2}+Q^{2}}+Q}{\left(\sqrt{4m_{N}^{2}+Q^{2}}+Q\right)^{2}}|G_{A}(Q^{2})|\left(\Delta|G_{M}^{n}(Q^{2})|\right)
\end{eqnarray}
\end{widetext}
to account for the uncertainty due to $G_{A}(Q^{2})$, $G_{M}^{p}(Q^{2})$
and $G_{M}^{n}(Q^{2})$ respectively. These three pieces are added
up in quadrature to obtain a total uncertainty:
\begin{equation}
\delta=\sqrt{\delta_1^2+\delta_2^2+\delta_3^2}.
\end{equation}

Due to the limitation of available data, in the numerical evaluation we integrate $Q^2$ up to $10$ GeV$^{2}$, which is practically equivalent to setting $Q_{\mathrm{max}}\rightarrow\infty$. The resulting central value is $1.05\times 10^{-3}$, with $\delta_1=4.9\times 10^{-5}$,
$\delta_2=1.5\times 10^{-5}$ and $\delta_3=2.7\times 10^{-5}$,
so the full result is $(1.05\pm 0.06)\times 10^{-3}$ as shown in Eq. \eqref{eq:Bornvalue}.


==> appcrossing.tex <==
In this appendix we demonstrate the crossing symmetry of the $\gamma W$ P-odd invariant function: $T_3^{(I)}(-\nu,Q^2)=\xi^I T_3^{(I)}(\nu,Q^2)$ where $\xi^{(0)}=-1$ and $\xi^{(3)}=1$. This relation is crucial in obtaining their dispersive representation \eqref{eq:DR}. Our derivation makes use of the following time-reversal identity:
\begin{equation}
\bigl\langle\beta\bigl|\hat{O}\bigr|\alpha\bigr\rangle=\bigl\langle\tilde{\alpha}\bigl|\mathbb{T}\hat{O}^{\dagger}\mathbb{T}^{-1}\bigr|\tilde{\beta}\bigr\rangle\label{eq:TReversal}
\end{equation}
where $\hat{O}$ is a linear operator, $\mathbb{T}$ is the time-reversal operator and $\bigl|\tilde{\alpha}\bigr\rangle=\mathbb{T}\bigl|\alpha\bigr\rangle$, $\bigl|\tilde{\beta}\bigr\rangle=\mathbb{T}\bigl|\beta\bigr\rangle$ are the time-reversed state. It is convenient to also define the time-reversed four-momentum: $\tilde{p}^\mu=p_\mu$ and recall the time-reversal operation to a four-current: 
\begin{equation}
\mathbb{T}J^\mu(\vec{x},t)\mathbb{T}^{-1}=J_\mu(\vec{x},-t).\label{eq:TJmu}
\end{equation} 

Now we may decompose the electromagnetic current into isoscalar and isovector components $J_{em}^\mu=J_{em}^{(0)\mu}+J_{em}^{(3)\mu}$ and compute their corresponding $V\times A$ component of the forward Compton tensor \eqref{eq:Compton} with $q\rightarrow -q$:
\begin{widetext}
\begin{eqnarray}
T_{\gamma W,VA}^{(I)\mu\nu}(p,-q)=\frac{1}{2}\int dxe^{iq\cdot x}\langle p(p)|T[\left(J^{\nu}_W(x)\right)_AJ^{(I)\mu}_{em}(0)]|n(p)\rangle
=\frac{1}{2}\int dxe^{i\tilde{q}\cdot x}\langle n(\tilde{p})|T[J^{em(I)}_{\mu}(x)\left(J^{W}_{\nu}(0)\right)^\dagger_A]|p(\tilde{p})\rangle\nn\\\label{eq:Tpminusq}
\end{eqnarray}
\end{widetext}
where the first equality is due to translational invariance and the second equality makes use of Eqs. \eqref{eq:TReversal}, \eqref{eq:TJmu} and the translational invariance. Next, we can prove the following identity:
\beqn
&&\langle n(\tilde{p})|T[J^{em(I)}_{\mu}(x)\left(J^{W}_{\nu}(0)\right)^\dagger_A]|p(\tilde{p})\rangle\nn\\
&&=-\xi^I \langle p(\tilde{p})|T[J^{em(I)}_{\mu}(x)\left(J^{W}_{\nu}(0)\right)_A]|n(\tilde{p})\rangle
\eeqn
straightforwardly using the Wigner-Eckart theorem in the isospin space. With these, we can now express both the LHS and RHS of Eq. \eqref{eq:Tpminusq} in terms of invariant function $T_3^{(I)}$ to get:
\beqn
&&\frac{i\epsilon^{\mu\nu\alpha\beta}p_\alpha q_\beta}{2(p\cdot q)}T_3^{(I)}\left(-\frac{p\cdot q}{M},Q^2\right)\nn\\
&&=-\xi^I\frac{i\epsilon_{\mu\nu\alpha\beta}\tilde{p}^\alpha\tilde{q}^\beta}{2(\tilde{p}\cdot \tilde{q})}T_3^{(I)}\left(\frac{\tilde{p}\cdot\tilde{q}}{M},Q^2\right).
\eeqn
Finally, using $\epsilon_{\mu\nu\alpha\beta}\tilde{p}^\alpha\tilde{q}^\beta=-\epsilon^{\mu\nu\alpha\beta}p_\alpha q_\beta$ and $\tilde{p}\cdot\tilde{q}=p\cdot q$, we immediately obtain the desired crossing symmetry relation $T_3^{(I)}(-\nu,Q^2)=\xi^I T_3^{(I)}(\nu,Q^2)$. 


==> apppiN.tex <==
\begin{figure}
\includegraphics[width=3.5cm]{loop1.pdf}
\includegraphics[width=3.5cm]{loop2.pdf}
\includegraphics[width=3.5cm]{loop3.pdf}
\includegraphics[width=3.5cm]{loop4.pdf}
\includegraphics[width=3.5cm]{loop5.pdf}
\includegraphics[width=3.5cm]{loop6.pdf}
\caption{Diagrams for $\pi N$ contribution to $F_3^{(0)}$.}
\label{fig:piN}
\end{figure}

Here we present the explicit result for the $\pi N$ contribution to the structure function $F_3^{(0)}(\nu,Q^2)$. It may be written as a sum of six terms coming from the discontinuity of the six one-loop diagrams depicted in Fig. \ref{fig:piN} respectively (which is also equivalent to calculating $M(nW\rightarrow N\pi)M^*(N\pi\rightarrow p\gamma)$ at tree level and integrating over the phase space):
\begin{equation}
F_{3,\, \pi N}^{(0)}=\sum_{i=1}^6 F_{3,i}^{{(0)}\pi N}.
\end{equation}
They are calculated using relativistic baryon chiral perturbation theory (ChPT) at leading order, keeping in mind that the photon is coupled to the isosinglet electromagnetic current, which leads to slight modifications of the corresponding Feynman rules; alternatively one could also calculate $F_{3,\gamma Z}^p-F_{3,\gamma Z}^n$ with the full Feynman rules, as shown in Section \ref{sec:relationtodata}.

The results are:
\begin{widetext}
\begin{eqnarray}
F_{3,1}^{{(0)}\pi N}&=&-\frac{g_AM\nu(M^4-M^2 m_\pi^2-2M^2W^2-m_\pi^2W^2+W^4)(E_+-E_-)}{64\pi^2 F_\pi^2W^2(W^2-M^2)q}\\
F_{3,2}^{{(0)}\pi N}&=&\frac{3g_A^3M\nu(M^6-M^4 m_\pi^2-(M^4+6M^2m_\pi^2)W^2-(M^2+m_\pi^2)W^4+W^6)(E_+-E_-)}{256\pi^2 F_\pi^2W^2(W^2-M^2)^2q}\\
F_{3,3}^{{(0)}\pi N} & = & -\frac{g_{A}^{3}\nu}{512\pi^{2}F_{\pi}^{2}q^{3}(W^{2}-M^{2})}\left\{ \left[4M^{2}W^{2}\left(2M^{4}+(2M^{2}+Q^{2})(W^{2}+Q^{2}-m_{\pi}^{2})+Q^{2}W^{2}\right)\right.\right.\nonumber\\
&  & \left.-(M^{2}+W^{2})(M^{2}+Q^{2}+W^{2})^{2}(W^{2}+M^{2}-m_{\pi}^{2})\right]\frac{E_{+}-E_{-}}{2MW^{2}}-\left[M^{6}\right.\nonumber\\
&  & +M^{4}(-2m_{\pi}^{2}+Q^{2}-W^{2})+M^{2}W^{2}(4m_{\pi}^{2}-2Q^{2}-W^{2})-2m_{\pi}^{4}Q^{2}-2m_{\pi}^{2}W^{4}\nonumber\\
&  & \left.\left.+W^{4}(Q^{2}+W^{2})\right]\ln\Xi\right\}\\
F_{3,4}^{{(0)}\pi N} & = & -\frac{g_{A}\nu}{128\pi^{2}F_{\pi}^{2}q^{3}}\left\{ \left[4M^{2}W^{2}(2M^{2}-m_{\pi}^{2}+Q^{2})\right.\right.\nonumber\\
&  & \left.-(M^{2}+Q^{2}+W^{2})^{2}(W^{2}+M^{2}-m_{\pi}^{2})\right]\frac{E_{+}-E_{-}}{2MW^{2}}-\left[M^{4}-M^{2}(Q^{2}+2W^{2})\right.\nonumber\\
&  & \left.\left.+2m_{\pi}^{2}Q^{2}+W^{2}(Q^{2}+W^{2})\right]\ln\Xi\right\}\nn\\
F_{3,5}^{{(0)}\pi N} & = & \frac{3g_{A}^{3}\nu}{512\pi^{2}F_{\pi}^{2}q^{3}(W^{2}-M^{2})}\left\{ \left[4M^{2}W^{2}\left(2M^{4}+2M^{2}(Q^{2}+W^{2})+m_{\pi}^{2}(Q^{2}-2W^{2})\right.\right.\right.\nonumber\\
&  & \left.\left.+Q^{4}+2Q^{2}W^{2}\right)-(M^{2}+W^{2})(M^{2}+Q^{2}+W^{2})^{2}(W^{2}+M^{2}-m_{\pi}^{2})\right]\frac{E_{+}-E_{-}}{2MW^{2}}\nonumber\\
&  & -\left[M^{6}+M^{4}(Q^{2}-W^{2})-M^{2}(2m_{\pi}^{2}Q^{2}+2W^{2}Q^{2}+W^{4})+2m_{\pi}^{4}Q^{2}+2m_{\pi}^{2}Q^{2}W^{2}\right.\nonumber\\
&  & \left.\left.+W^{4}(Q^{2}+W^{2})\right]\ln\Xi\right\}\nonumber\\
F_{3,6}^{{(0)}\pi N} & = & \frac{g_{A}^{3}\nu}{512\pi^{2}F_{\pi}^{2}q^{3}}\left\{ \left[\left(4M^{2}W^{2}-(M^{2}+Q^{2}+W^{2})^{2}\right)\left(W^{2}+M^{2}-m_{\pi}^{2}\right)\right.\right.\nonumber\\
&  & \left.-\frac{8M^{2}m_{\pi}^{2}Q^{2}W^{4}\left(-3M^{2}+2m_{\pi}^{2}-Q^{2}-W^{2}\right)}{M^{6}-2M^{4}W^{2}+M^{2}(3m_{\pi}^{2}Q^{2}+W^{4})+m_{\pi}^{2}Q^{2}(W^{2}+Q^{2}-m_{\pi}^{2})}\right]\frac{E_{+}-E_{-}}{2MW^{2}}\nonumber\\
&  & \left.+2m_{\pi}^{2}\left(M^{2}+Q^{2}-W^{2}\right)\ln\Xi\right\} 
\end{eqnarray}
\end{widetext}
where $\lambda(a,b,c)=a^2+b^2+c^2-2ab-2bc-2ca$ is the usual  K\"{a}ll\'{e}n function, $E_\pm$ is the maximum and minimum energy of nucleon in an $N\pi$-final state:
	\beqn
	E_\pm&=&\frac{(W^2+M^2+Q^2)(W^2+M^2-m_\pi^2)}{4MW^2}\nn\\
	&\pm&\frac{q\lambda^{\frac{1}{2}}(M^2,m_\pi^2,W^2)}{2W^2}
	\eeqn
	and 
		\begin{equation}
		\ln \Xi=\ln \left(\frac{2ME_+-M^2+m_\pi^2-Q^2-W^2}{2ME_--M^2+m_\pi^2-Q^2-W^2}\right)
		\end{equation}
is a frequently-appearing logarithmic function.

It is well-known that ChPT is an effective field theory at low energy, so the results above apply only at low $Q^2$; in particular, it clearly overestimated the size of $N\pi$ effects at large $Q^2$. Form factors may be supplemented to suppress large-$Q^2$ contributions, but they should be added in a way to preserve the vector and axial current conservation:
\begin{equation}
q_\mu\left\langle p\right|J_{em}^{(0)\mu}\left|N\pi\right\rangle=0\:\:\:,\:\:\:\lim_{m_\pi\rightarrow 0}q_\mu\left\langle N\pi\right|\left(J_{W}^{\mu}\right)_A\left|n\right\rangle=0.
\end{equation} 
Here we choose to multiply our ChPT result by the isosinglet electromagnetic form factor $F_1^S(Q^2)$ and the axial form factor $-g_A^{-1}G_A(Q^2)$, which is a natural extension of the na\"{\i}ve Feynman rules applied in the ChPT calculation. 

With these results at hand, we can check the assumption of Ref. \cite{Marciano:2005ec} that chiral symmetry requires $F(Q^2=0)=0$. 
\begin{figure}[h]
\includegraphics[width=8cm]{SCR_ChPT.pdf}
\caption{The integrand of $F_3^{(0)\pi N}(\nu_\pi/z,0)$ }
\label{fig:SCR}
\end{figure}
This condition translates in the following superconvergence relation,
\beqn
\int_{\nu_\pi}^\infty\frac{d\nu}{\nu^2}F_{3,\, \pi N}^{(0)}(\nu,0)=0.
\eeqn
We find that this relation does not hold. To visualize it, we plot $F_3^{(0)\pi N}(\nu,0)$ as function of $z=\nu_\pi/\nu$ for which the integral in question becomes simply $\int_0^1 dzF_3^{(0)\pi N}(\nu_\pi/z,0)$ in the full range of the variable $z\in(0,1)$ in Fig. \ref{fig:SCR}. It is obvious that the surface below and above the curve are not equal and the integral does not vanish.

Finally, the $N\pi$-final state contributions to the $\nu p$ and $\bar{\nu}p$ scattering can also be calculated in the same manner, except that there is an extra $\pi\pi W$ vertex coming from the vector part of the charged weak current. The calculation thus involve more Feynman diagrams and we choose not to present it here. 


==> appregge.tex <==

In this appendix we show in detail how we obtain data input to the Regge contribution to the $\gamma W$-box from the inclusive $\nu p$ and $\bar{\nu} p$-scattering. 

The main objects of study are the P-odd structure functions $F_3^{(0)}$ and $F_3^{\nu p+\bar{\nu}p}$, and we will show that they are proportional to each other in the framework of Regge model with vector (axial vector) meson dominance. The physical picture is the following: in the VDM, the two energetic and slightly virtual gauge bosons fluctuate into a vector/axial-vector meson. The transition between the initial and final state proceeds via a $t$-channel exchange of a mesonic Regge trajectory with appropriate quantum numbers. 

The mechanism described above is depicted in Fig. \ref{fig:Regge}. The structure function $F_3^{(0)}$ involves the product between the isosinglet component of the electromagnetic current and the axial component of the charged weak current. Then, the $W$-boson should fluctuate into an isovector axial meson $a_1$ while the  isoscalar photon should fluctuate into an  isoscalar vector meson $\omega$. The exchanged meson in the $t$-channel should be the isotriplet vector meson $\rho$ in order to conserve isospin. Meanwhile, the three-meson vertex responsible for $F_3^{\nu p+\bar{\nu}p}$ is also $a_1\omega\rho$, except that this time the currents are the vector and axial components of the charged weak current, so the W-bosons should fluctuate into $\rho$ and $a_1$, respectively, whereas the exchanged-meson in the $t$-channel is $\omega$. The relevant gauge boson-vector meson mixing Lagrangian can be written as \cite{Lichard:1997ya}:
\beqn
\mathcal{L}_{\mathrm{VDM}}&=&\left(\frac{em_\rho^2}{g_\rho}\rho_\mu^0+\frac{em_\omega^2}{g_\omega}\omega_\mu\right) A^\mu\nn\\
&+&\frac{gm_\rho^2}{2g_\rho}V_{ud}\left(W_\mu^-\rho^{+\mu}+h.c.\right)\nn\\
&-&\frac{gm_{a_1}^2}{2g_{\rho}}w_{a_1}V_{ud}\left(a_{1\mu}^+W^{-\mu}+h.c.\right)
\eeqn
with the assumption that $g_{\omega}=3g_\rho$ following static SU(6) prediction \cite{deSwart:1963pdg}. Correspondingly, the vector meson coupling to nucleon is:
\begin{equation}
\mathcal{L}_{NNV}=\frac{g_\rho}{2}\bar{N}\gamma^\mu\vec{\tau}\cdot\vec{\rho}_\mu N+\frac{g_\omega}{2}\bar{N}\gamma^\mu \omega_\mu N.
\end{equation}
Note that the coupling strengths $g_\rho$ and $g_\omega$ appeared are the same as those in the mixing Lagrangian $\mathcal{L}_\mathrm{VDM}$ as a consequence of the universality relation within the VDM framework. Finally, one may write down a phenomenological $\rho-\omega-a_1$ interaction Lagrangian with two independent operators:
\begin{equation}
\mathcal{L}_{\rho\omega a_1}=g_1\epsilon^{\mu\nu\alpha\beta}(\partial_\mu\omega_\nu)\rho^i_\alpha a_{1\beta}^i+g_2\epsilon^{\mu\nu\alpha\beta}(\partial_\mu\rho^i_\nu)\omega_\alpha a_{1\beta}^i.
\end{equation}
It is obvious that the first operator only contributes to $F_3^{(0)}$ whereas the second operator only contributes to $F_3^{\nu p}$ and $F_3^{\bar{\nu}p}$ because there is no momentum exchange in the t-channel. We will further assume the exact equality of the two coupling constants $g_1,g_2$ as suggested in \cite{Harvey:2007rd} that comes from large-$N_c$ expansion, and will see that this is an important relation that leads to the near-degeneracy between the first Nachtmann moment of the Regge-induced $F_3^{(0)}$ and $F_3^{\nu p+\bar{\nu}p}$. 

With the ingredients above we may now proceed to write down the general form of the Regge contribution to $F_3^{(0)}$ and $F_3^{\nu p}$:
\begin{widetext}
\begin{eqnarray}
F_{3,\,\mathbb{R}}^{(0)}(\nu,Q^2)&=&\frac{1}{2}\left(\frac{eg}{2\sqrt{2}}V_{ud}\right)^{-1}\left(\frac{e}{g_\omega}\frac{m_\omega^2}{m_\omega^2+Q^2}\right)\left(-\frac{g}{2g_{\rho}}w_{a_1}V_{ud}\frac{m_{a_1}^2}{m_{a_1}^2+Q^2}\right)\left(\frac{g_\rho}{\sqrt{2}}\right)g_1H_\rho(\nu,Q^2)\nonumber\\
F_{3,\,\mathbb{R}}^{\nu p}(\nu,Q^2)&=&2\left(-\frac{g}{2\sqrt{2}}V_{ud}\right)^{-2}\left(\frac{g}{2g_\rho}V_{ud}\frac{m_\rho^2}{m_\rho^2+Q^2}\right)\left(-\frac{g}{2g_{\rho}}w_{a_1}V_{ud}\frac{m_{a_1}^2}{m_{a_1}^2+Q^2}\right)\left(\frac{g_\omega}{2}\right)g_2H_\omega(\nu,Q^2)\label{eq:F3Regge}
\end{eqnarray}
\end{widetext}
Notice the existence of the factor 1/2 and 2 in front of $F_{3,\,\mathbb{R}}^{(0)}$ and $F_{3,\,\mathbb{R}}^{\nu p}$ respectively; the first factor is due to our definition of $W_{\gamma W}^{\mu\nu}$ that contains a prefactor of $1/(8\pi)$ instead of $1/(4\pi)$; whereas the second factor is because $a_1$ can either couple to the incoming or outgoing $W$-boson in $F_{3,\,\mathbb{R}}^{\nu p}$. The function $H_V(\nu,Q^2)$ ($V=\rho,\omega$) encodes the information of the Regge-trajectory as well as all other universal multiplicative factors. From a pure Regge point of view one should expect $H_\rho(\nu,Q^2)\approx H_{\omega}(\nu,Q^2)$ due to the almost degenerate trajectories of $\rho$ and $\omega$; but here we may allow them to be different in order to account for other physics that could break such universality. The Regge contribution to $F_3^{\bar{\nu}p}$ can be calculated accordingly and it turns out to be identical to $F_{3,\mathbb{R}}^{\nu p}$. Upon setting $g_\omega=3g_\rho$ and $g_2=g_1$ and approximating $m_\omega\approx m_\rho$, one observes the following ratio: 
\begin{equation}
\frac{F_{3,\,\mathbb{R}}^{\nu p+\bar{\nu}p}(\nu,Q^2)}{F_{3,\,\mathbb{R}}^{(0)}(\nu,Q^2)}\approx \frac{36H_\omega(\nu,Q^2)}{H_\rho(\nu,Q^2)}.\label{eq:F3ratio}
\end{equation} 

One may now parameterize the first Nachtmann moment of both the $F_3$ functions as follows:
\begin{eqnarray}
&&M_{3,\,\mathbb{R}}^{(0)}(1,Q^2)=\frac{m_\omega^2}{m_\omega^2+Q^2}\frac{m_{a_1}^2}{m_{a_1}^2+Q^2}Q^2G_\rho(Q^2)\label{eq:M3parameter}\\
&&M_{3,\,\mathbb{R}}^{\nu p+\bar{\nu}p}(1,Q^2)=36\frac{m_\rho^2}{m_\rho^2+Q^2}\frac{m_{a_1}^2}{m_{a_1}^2+Q^2}Q^2G_\omega(Q^2).\nn
\end{eqnarray} 
A few explanations: (1) we retain the vector meson propagators as they are untouched by the integration over $\nu$; (2) we include an explicit factor of $Q^2$ in the parameterization to emphasize the fact that by definition the first Nachtmann moments vanish as $Q^2$ when $Q^2\rightarrow 0$, and (3) the explicit factor of 36 in $M_3^{\nu p+\bar{\nu}p}$ reflects the ratio in Eq. \eqref{eq:F3ratio}. 

We may now investigate the relation between the two functions $G_\rho(Q^2)$ and $G_\omega(Q^2)$ through a few matching conditions. First, it is natural to assume that $H_\omega(\nu,Q^2)$ and $H_\rho(\nu,Q^2)$ equal each other in the $Q^2\rightarrow 0$ limit, which reflects our belief that the VDM+Regge picture does appropriately describe the physics at low $Q^2$; that implies the constraint $G_\rho(0)=G_\omega(0)$. Second, we require the Regge prediction to smoothly match the perturbative QCD prediction at some matching value of $Q^2$. Recall that in the partonic description both the P-odd structure functions can be expressed in terms of valence quark PDFs of proton: $F_3^{(0)}(x)=(1/24)u_V^p(x)$ (as discussed in Appendix \ref{app:DIS}) and $F_3^{\nu p+\bar{\nu}p}=u_V^p(x)+d_V^p(x)$, which means their first Mellin's moments obey the following sum rules in the $Q^2\rightarrow \infty$ limit:
\begin{equation}
\int_0^1dx F_3^{(0)}(x)=\frac{1}{12}\:\:\:,\:\:\:\int_0^1dxF_3^{\nu p+\bar{\nu}p}(x)=3.
\end{equation}
In particular, the second line is just the GLS sum rule. At finite $Q^2$ both expressions are modified by pQCD. As pointed out in Ref. \cite{Marciano:2005ec}, the pQCD correction to the first equation follows that of the Bjorken sum rule for polarized electroproduction, which turns out to be identical to that of the GLS sum rule up to very small corrections of order $(\alpha_s/\pi)^3$ \cite{Larin:1991tj}. In other words, the ratio
\begin{equation}
\frac{\int_0^1dxF_3^{\nu p+\bar{\nu}p}(x)}{\int_0^1dx F_3^{(0)}(x)}=36\label{eq:pdfratio}
\end{equation} 
is stable with respect to pQCD corrections. As the first Nachtmann moment reduces to the first Mellin's moment at large $Q^2$, our second matching condition is to require this ratio to be satisfied by $M_3^{(0)}(Q^2)/M_3^{\nu p+\bar{\nu}p}(Q^2)$ at some matching point $Q^2=Q_0^2$.

Consider for instance a simple parameterization of $G_i(Q^2)$ with two free parameters: $G_i(Q^2)=F(a_i,b_i,Q^2)$. For $i=\omega$, the parameters can be fitted to existing experimental data of the GLS sum rule after subtracting out the elastic, $N\pi$ and resonance contributions by hand. Meanwhile, through the inspection of Eq. \eqref{eq:M3parameter} and \eqref{eq:pdfratio}, one immediately finds that upon approximating $m_\rho\approx m_\omega$, the two matching conditions simply imply $F(a_\omega,b_\omega,0)=F(a_\rho,b_\rho,0)$ and $F(a_\omega,b_\omega,Q_0^2)=F(a_\rho,b_\rho,Q_0^2)$, and the most natural solution is $a_\omega=a_\rho$, $b_\omega=b_\rho$, i.e. $G_\rho(Q^2)=G_\omega(Q^2)$. The key feature that leads to this conclusion is the existence of the same relative factor 36 in both equations: in Eq. \eqref{eq:M3parameter} this factor results from the model-predicted relations among $\{g_\rho,g_\omega\}$ as well as $\{g_1,g_2\}$ that are expected to hold at low $Q^2$, whereas in Eq. \eqref{eq:pdfratio} it is just a parton-model prediction which works at large $Q^2$. Such an agreement between two predictions at very different $Q^2$ suggests that it is reasonable to regard $M_3^{\nu p+\bar{\nu}p}(1,Q^2)$ and $M_3^{(0)}(1,Q^2)$ as being proportional to each other. Then, we extract the former from neutrino scattering data and divide it by 36 to obtain the later. Despite of lack of direct experimental data, this straightforward procedure provides the first solid and data-driven prediction for the Regge contribution to $\gamma W$ box diagram.


==> appresonances.tex <==

Next we consider the effects of a baryon resonance $R$ to $\Box_{\gamma W}^{VA}$. We first observe that since only the isoscalar component of the electromagnetic current is involved, the contributing resonances must have isospin-1/2. This immediately gets rid of all isospin-3/2 resonances including the $\Delta$s which are usually the main contributors in the resonance region. For practical purpose we assume that the resonance $R$ takes the Breit-Wigner form with mass $m_R$ and width $\Gamma_R$. With these, the resonance contribution to $F_3^{(0)}$ is given by:
\beqn
F_{3,\,\rm res}^{(0)}&=&\sum_R\frac{\frac{\nu}{q}\Gamma_Rm_R}{(W^2-m_R^2)^2+\Gamma_R^2m_R^2}\sqrt{\frac{M(m_R^2-M^2)}{16\pi^3\alpha}}\nn\\
&\times&\sum_{J_z=1/2,3/2}(A_{em,J_z}^{R,p}+A_{em,J_z}^{R,n})^*A_{w,J_z}^R
\eeqn
where 
\begin{eqnarray}
A_{em,1/2}^{R,N} & = & -\sqrt{\frac{\pi\alpha}{M(m_{R}^{2}-M^{2})}}\left\langle R,+\frac{1}{2}\right|J_{em}^{+}\left|N,-\frac{1}{2}\right\rangle \nonumber \\
A_{em,3/2}^{R,N} & = & -\sqrt{\frac{\pi\alpha}{M(m_{R}^{2}-M^{2})}}\left\langle R,+\frac{3}{2}\right|J_{em}^{+}\left|N,+\frac{1}{2}\right\rangle \nn\\
\end{eqnarray}
are the standard electromagnetic transverse helicity amplitudes for the resonance $R$; the transverse components of the electromagnetic current are defined as $J_{em}^\pm=\mp (1/\sqrt{2})(J_{em}^x\pm iJ_{em}^y)$. In principle,
there is a sign ambiguity in the definition of the helicity amplitude,
which is related to the choice of sign for the $R\rightarrow N\pi$
coupling; throughout the paper we shall choose the same sign convention
as in Ref. \cite{Lalakulich:2006sw}. The transverse helicity amplitudes of the axial charged weak current are similarly defined as:
\beqn
A_{w,1/2}^R&=&\left\langle R,+\frac{1}{2}\right|\left(J_{w}^{+}\right)_A\left|n,-\frac{1}{2}\right\rangle,\nn\\
A_{w,3/2}^R&=&\left\langle R,+\frac{3}{2}\right|\left(J_{w}^{+}\right)_A\left|n,+\frac{1}{2}\right\rangle.
\eeqn

The values of the electromagnetic helicity amplitudes $A_{em,1/2}^{R,N},A_{em,3/2}^{R,N}$ in the vicinity of $Q^2=0$ can be obtained from partial wave analyses of $\pi,\eta$ photo- and electro-production; however for the evaluation of the dispersion integral their full $Q^2$-dependence is required and thus inputs from models are unavoidable at this point. In this work their functional form are taken from the unitary isobar model MAID2007 \cite{Drechsel:2007if,Tiator:2008kd}. In the meantime, there are much less studies of the transition matrix elements of the axial charged current. Here we make use of results of Ref. \cite{Lalakulich:2006sw} in which axial transition matrix elements of the lowest-lying spin-1/2 and 3/2 resonances at $Q^2=0$ are inferred from the $R\rightarrow N\pi$ decay width, and a modified dipole form is assumed for their $Q^2$-dependence. 

Applying the parameterizations in Ref. \cite{Drechsel:2007if,Tiator:2008kd,Lalakulich:2006sw}, we study the effects of the few lowest-lying $N^*$ resonances: $P_{11}(1440)$, $S_{11}(1535)$, $D_{13}(1520)$ and $S_{11}(1650)$, and find that their contributions to $\Box_{\gamma W}^{VA}$ are generally of the order $10^{-7}-10^{-5}$ which are negligibly small. This can be partially understood as due to the smallness of the isosinglet electromagnetic transition matrix element $A_{em}^{R,p}+A_{em}^{R,n}$ because the isosinglet component of the electromagnetic current is by itself small. Thus, we conclude that it is safe to disregard the contributions from discrete resonances and focus on the continuum. 

In the meantime, in order to extract the Regge piece in the inclusive neutrino scattering data, resonance contributions must be subtracted out by hand so we shall calculate the latter in the same manner. The main difference is, however, that in this case the resonances can have either $I=1/2$ or $3/2$; therefore the contribution from $\Delta$ is obviously the dominant piece so it is sufficient to consider only this piece. Also, according to isospin symmetry one has $F_{3,\Delta}^{\bar{\nu}p}=(1/3)F_{3,\Delta}^{\nu p}$ and therefore $F_{3,\Delta}^{\nu p+\bar{\nu}p}=(2/3)F_{3,\Delta}^{\nu p}$. Extensive model study of the $N-\Delta$ matrix element of charged weak current can be found in Ref. \cite{Lalakulich:2005cs} so here we simply quote their results relevant to our work after taking into account all differences in conventions:
\begin{equation}
F_{3,\Delta}^{\nu p+\bar{\nu}p}=-\frac{2\nu}{M}\frac{m_\Delta \Gamma_\Delta}{\pi}\frac{1}{(W^2-m_\Delta^2)^2+m_\Delta^2\Gamma_\Delta^2}\frac{V_3}{3}
\end{equation}
where 
\begin{eqnarray}
\frac{V_3}{3}&=&\frac{4}{3m_\Delta}\left[-\frac{C_3^VC_4^A}{M}(M\nu-Q^2)-C_3^VC_5^AM\right]\\
&\times&\left[2m_\Delta^2+2Mm_\Delta+Q^2-M\nu\right]\nonumber\\
&+&\frac{4}{3}\left[M\nu-Q^2\right]\left[-\frac{C_4^VC_4^A}{M^2}(M\nu-Q^2)-C_4^VC_5^A\right]\nn
\end{eqnarray}
and $m_\Delta$, $\Gamma_\Delta$ are the mass and width of the $\Delta$-resonance respectively. The $C$-functions are parameterized as:
\begin{eqnarray}
C_3^V&=&\frac{1.95}{\left(1+\frac{Q^2}{m_V^2}\right)^2}\frac{1}{1+\frac{Q^2}{4m_V^2}}\nonumber\\
C_4^V&=&-C_3^V\frac{M}{\sqrt{W^2}}\nonumber\\
C_5^A&=&\frac{1.2}{\left(1+\frac{Q^2}{m_A^2}\right)^2}\frac{1}{1+\frac{Q^2}{3m_A^2}}\nonumber\\
C_4^A&=&-\frac{C_5^A}{4}
\end{eqnarray}
where $m_V=0.84$GeV and $m_A=1.05$GeV.
